Erasure Broadcast Channels with Intermittent Feedback

Achievable data rates in wireless systems rely heavily on the available channel state information (CSI) throughout the network. However, feedback links, which provide this information, are scarce, unreliable, and subject to security threats. In this work, we study the impact of having intermittent feedback links on the capacity region of the canonical two-user erasure broadcast channels. In our model, at any time instant, each receiver broadcasts its CSI, and at any other node, this information either becomes available with unit delay or gets erased. For this setting, we develop a new set of outer bounds to capture the intermittent nature of the feedback links. These outer bounds depend on the probability that the CSI from both receivers are erased at the transmitter. In particular, if at any time, the CSI from at least one of the two receivers is available at the other two nodes, then the outer-bounds match the capacity with global delayed CSI. We also provide capacity-achieving transmission strategies under certain scenarios, and we establish a connection between this problem and Blind Index Coding with feedback.

==> Achievability_IFB_symmetric.tex <==
We start from the achievability of Case~1, which is a review of our previous work \cite{ISIT19sclin}, and then present the new achievability for the other two cases.

\noindent {\bf Case~1}: If $\delta_{F1} = 0$ and $\delta_{F2} = 0$, then the capacity region of the two-user BC with intermittent FB is equivalent to that of global delayed CSI assumption (or ``DD'' assumption)~\cite{GeorgiadisDetDelayedBC}. Note that based on (\ref{Eq:deltadefinitions}), $\delta_{Fi} = 0$, $i=1,2$, means feedback links originating at ${\sf Rx}_i$ are always active and no erasure happens to the feedback signal of that receiver. 

On the other hand, if one of the $\delta_{Fi}$'s is non-zero, then the capacity includes that of a two-user erasure BC with one-sided feedback (``DN'' assumption) for which we recently proved the capacity region coincides with that of DD assumption~\cite{ISIT19sclin}. 

\begin{figure}[!ht]
\centering
\includegraphics[width = \columnwidth]{FiguresPDF/BC-DN.pdf}
\caption{A summary of the transmission protocol of~\cite{ISIT19sclin} with one-sided delayed channel state information (``DN'' assumption): during Phase 1, the transmitter learns which bits are missing at ${\sf Rx}_1$, and creates $v_{1|2}^{\mathrm{noFB}}$, which is of interest to ${\sf Rx}_1$ and \underline{partially} known at ${\sf Rx}_2$. The ``$\mathrm{noFB}$'' superscript indicates lack of feedback from ${\sf Rx}_2$; during the second phase, the transmitter learns which bits are delivered to the unintended receiver and creates $v_{2|1}^{\mathrm{FB}}$, which is of interest to ${\sf Rx}_2$ and \underline{fully} known at ${\sf Rx}_1$.\label{Fig:DN}}
\end{figure}

Here, we include a very brief overview of the achievability strategy under the DN assumption, both for the completeness of the current paper and for our discussion later in Section~\ref{Section:Discussion_IFB}. In the DN scenario, suppose only receiver 1 provides its feedback and receiver 2 is always silent. Furthermore, there is no erasure possibility and the CSI of receiver 1 is available to the other nodes with unit delay. The transmission strategy includes three phases as illustrated in Fig.~\ref{Fig:DN}. During the first phase, the transmitter communicates the bits intended for ${\sf Rx}_1$ and through the one-sided feedback learns which bits are missing at ${\sf Rx}_1$. A fraction $(1-\delta_2)$ of these bits are available at ${\sf Rx}_2$. During the second phase, the transmitter communicates the bits intended for ${\sf Rx}_2$ and through the one-sided feedback learns which bits are delivered to the unintended receiver, \emph{i.e.} ${\sf Rx}_1$. During the third phase, the transmitter sends out the XOR of the missing bits of Phase~1 and random linear combination of the bits delivered to the unintended receiver during Phase~2. Using feedback, when the missing bits are delivered to the intended receiver, a new bit joins the XOR process. Note that unlike prior results, feedback is utilizes during all three phases of communications in order to achieve the DD capacity. Details of this scheme are presented in~\cite{ISIT19sclin}. 

% {\bf Shih-Chun please revise this part as you wish.}

\noindent {\bf Case~2}: $\delta_{F1} = \delta_{F2} \overset{\triangle}= \delta_F$ and $\Pr\left( S_{F1T}[t] \neq S_{F2T}[t] \right) = 0$. This also implies that $\delta_{FF} = \delta_F$ since we also have $S_{F_iT}[t]=S_{F_{i\bar{i}}}[t], i=1,2$. Moreover, we have $\delta_1 = \delta_2  \overset{\triangle}= \delta$.

In this case, we can simplify some expressions as follows.
\begin{align}
\label{Def:A}
\beta_i = \frac{(1-\delta_{12})-\delta_F(\delta-\delta_{12})}{1-\delta} \overset{\triangle}= \frac{A}{1-\delta}.
\end{align}
Then, from Theorem~\ref{THM:Capacity_IFB}, we obtain the maximum sum-rate corner point:
\begin{align}
\label{Eq:TargetRates}
R_1 = R_2 = \frac{A}{1+\frac{A}{(1-\delta)}}.
\end{align} 

\noindent {\bf Transmission Protocol}: The transmission strategy has a recursive format. We start with $m$ bits for each receiver. We start by sending the bits for each receiver and based on the available feedback, we create two sets of recycled equations. For the first set, feedback bits were available whereas for the second set, no feedback was available. We then send the XOR of the bits in first set. Whatever is left will be fed as the input to the transmission protocol again.


\noindent {\bf Phase~1}: The transmitter creates 
\begin{align}
\frac{m}{1-\delta_{12}}
\end{align}  
linearly independent equations of the $m$ bits for receiver $1$ and sends them out. For $(1-\delta_F)$ fraction of the time, feedback is available and 
\begin{align}
\label{Eq:Rx1FB}
(1-\delta_F) \frac{\delta-\delta_{12}}{1-\delta_{12}} m
\end{align} 
bits are available at ${\sf Rx}_2$ and needed at ${\sf Rx}_1$. Denote these bits by $v_{1|2}$. Moreover, for $\delta_F$ fraction of the time, no feedback is available. But due to the statistics of the channel, we know 
\begin{align}
\label{Eq:Rx1noFB}
\delta_F \frac{\delta-\delta_{12}}{1-\delta_{12}} m = \frac{\delta_F}{1-\delta_F} \left| v_{1|2} \right|
\end{align} 
bits are available at ${\sf Rx}_2$ and needed at ${\sf Rx}_1$. The transmitter creates the same number of linearly independent equations as (\ref{Eq:Rx1noFB}) from the transmitted bits $X[t]$ when feedback links were not available. Denote these equations by $v^{\mathrm{noFB}}_{1|2}$.

\begin{remark}
\label{remark:Bernstein}
To keep the description of the protocol simple, we use the expected value of the number of bits in different states, \emph{e.g.}, (\ref{Eq:Rx1FB}) and (\ref{Eq:Rx1noFB}). A more precise statement would use a concentration theorem result such as the Bernstein inequality to show the omitted terms do not affect the overall result and the achievable rates. A detailed example of such calculations can be found in Section V.B of~\cite{Vahid_IT16}. Moreover, when talking about the number of bits or equations, we are limited to integer numbers. If a ratio is not an integer number, we can use $\lceil \cdot \rceil$, the ceiling function, and since at the end we take the limit for $m \rightarrow \infty$, the results remain unchanged.
\end{remark}
%  as done in~\cite{vahid2014capacity,vahid2016two}

\noindent {\bf Phase~2}: This phase is similar to the previous one. The transmitter creates 
\begin{align}
\frac{m}{1-\delta_{12}}
\end{align}  
linearly independent equations of the $m$ bits for receiver $2$ and sends them out. For $(1-\delta_F)$ fraction of the time, feedback is available and 
\begin{align}
(1-\delta_F) \frac{\delta-\delta_{12}}{1-\delta_{12}} m
\end{align} 
bits are available at ${\sf Rx}_1$ and needed at ${\sf Rx}_2$. Denote these bits by $v_{2|1}$. Moreover, for $\delta_F$ fraction of the time, no feedback is available. But due to the statistics of the channel, we know 
\begin{align}
\label{Eq:Rx2noFB}
\delta_F \frac{\delta-\delta_{12}}{1-\delta_{12}} m = \frac{\delta_F}{1-\delta_F} \left| v_{2|1} \right|
\end{align} 
bits are available at ${\sf Rx}_1$ and needed at ${\sf Rx}_2$. The transmitter creates the same number of linearly independent equations as (\ref{Eq:Rx2noFB}) from the transmitted signal when feedback links were not available. Denote these equations by $v^{\mathrm{noFB}}_{2|1}$.

\noindent {\bf Phase~3}: In this phase, the transmitter encodes $v_{1|2}$ and $v_{2|1}$ using erasure codes of rate $(1-\delta)$. Note that $\left| v_{1|2} \right| = \left| v_{2|1} \right|$. The transmitter creates the XOR of the encoded bits for ${\sf Rx}_1$ and ${\sf Rx}_2$ and sends them out. This Phase takes  
\begin{align}
\frac{\left| v_{1|2} \right|}{(1-\delta)} = \frac{(1-\delta_F)(\delta-\delta_{12})}{(1-\delta)(1-\delta_{12})}m.
\end{align} 
time instants. 

\noindent {\bf Recursive step}: Consider $v^{\mathrm{noFB}}_{1|2}$ and $v^{\mathrm{noFB}}_{2|1}$ as the input messages in new Phase~1 and Phase~2, respectively, and repeat the communication strategy. 

\noindent {\bf Termination}: To simplify the protocol, when the remaining bits in $v^{\mathrm{noFB}}_{1|2}$ and $v^{\mathrm{noFB}}_{2|1}$ is $o\left( m^{1/3} \right)$ we stop the recursion and send the remaining bits using time sharing between the two erasure codes. Note that while we used $o\left( m^{1/3} \right)$ as our termination threshold, any threshold with vanishing (as $m \rightarrow \infty$) impact would work. 

\noindent {\bf Decoding}: Our transmission protocol is built upon that of global feedback~\cite{GeorgiadisDetDelayedBC,Wang_12,GatzianasGeorgiadis_13} with the addition of the recursive step. Decoding starts with the last recursive step and goes backwards to the first iteration. A subtle point worth noting is that in each iteration the transmitter creates linearly independent equations similar to $v^{\mathrm{noFB}}_{1|2}$ and $v^{\mathrm{noFB}}_{2|1}$, and we need to guarantee that this task is feasible as we have many iterations. It is easy to verify that the geometric sum of the number of linearly independent equations created for each receiver during all iterations is smaller than the total number of unknown bits we start with, \emph{i.e.} $m$. Thus, the transmitter is able to carry out its task as needed. 

\noindent {\bf Achievable rates}: Achievable rates are calculated as the ratio of the number of transmitted bits divided by the total communication time for $m \rightarrow \infty$ as below:
\begin{align}
\label{Eq:RatesCase2}
R_{\mathrm{SUM}} \overset{m \rightarrow \infty}= \frac{2m}{\frac{2 m}{1-\delta_{12}}+ \frac{(1-\delta_F)(\delta-\delta_{12})}{(1-\delta)(1-\delta_{12})} m + \frac{2 \left| \bar{v}^{\mathrm{noFB}}_{2|1} \right|}{R_{\mathrm{SUM}}}}.
\end{align}
where 
\begin{align}
\label{Eq:RatesCase2Exp}
\left| \bar{v}^{\mathrm{noFB}}_{2|1} \right| = \delta_F \frac{\delta-\delta_{12}}{1-\delta_{12}} m.
\end{align}
From~\eqref{Eq:RatesCase2} and~\eqref{Eq:RatesCase2Exp}, we have
\begin{align}
& R_{\mathrm{SUM}} \left( \frac{2}{1-\delta_{12}}+ \frac{(1-\delta_F)(\delta-\delta_{12})}{(1-\delta)(1-\delta_{12})} \right) = 2 - 2 \delta_F \frac{\delta-\delta_{12}}{1-\delta_{12}} \nonumber \\
& \Rightarrow R_{\mathrm{SUM}} = \frac{2A(1-\delta)}{2(1-\delta)+(1-\delta_F)(\delta-\delta_{12})},
\end{align}
where for the last equality, we used the definition of $A$ as given in~\eqref{Def:A}:
\begin{align}
A = (1-\delta_{12}) - \delta_F(\delta-\delta_{12}).
\end{align}

We can further rearrange the denominator of this equality as
\begin{align}
2(1-\delta)+(1-\delta_F)(\delta-\delta_{12}) = (1-\delta) + (1-\delta_{12}) - \delta_F(\delta-\delta_{12}) \overset{\eqref{Def:A}}= 1 -\delta + A,
\end{align}
to obtain
\begin{align}
R_{\mathrm{SUM}} = R_1 + R_2 = \frac{2A(1-\delta)}{(1-\delta+A)},
\end{align}
where $R_1$ and $R_2$ are given in (\ref{Eq:TargetRates}). This completes the avhievability proof of Case~2.

\begin{comment}

%ALIREZA


\noindent {\bf Case~3}: Recall that in Case~2, feedback links are fully correlated, \emph{i.e.} $\Pr\left( S_{F1T}[t] \neq S_{F2T}[t] \right) = 0$. In Case~3, on the other hand, we allow for a more general distribution of feedback links originating from different receivers. More specifically, feedback links from each receiver are still fully correlated, \emph{i.e.} $S_{F1T}[t] = S_{F12}[t]$ for $\msf{Rx}_1$ and vice versa, but feedback links originating from different receivers can have a more general distribution (unlike Case~2). We also assume all erasure links are governed by Bernoulli $(1 - \delta)$ random variables and $\delta_{FF} = \delta_{12} = \delta^2$. Fig.~\ref{Fig:FBCase3} depicts all possible feedback realizations and the corresponding probabilities. The non-trivial corner point based on Theorem~\ref{THM:Capacity_IFB} is given by
\begin{align}
\label{Eq:RSUMCase3}
R_1 = R_2 = \frac{\beta(1-\delta)}{1+\beta},
\end{align}
where
\begin{align}
\label{Def:beta-case3}
\delta_i = \delta_{F_i} = \delta, \delta_{12} = \delta_{FF} = \delta^2 \Rightarrow \beta_i = \beta = \frac{\delta_{12}(1-\delta)+(1-\delta_{12})^2}{(1-\delta)} \overset{\delta < 1}= 1+\delta-\delta^3.
\end{align}

\noindent {\bf Transmission Protocol (overview)}: We start with $m$ bits for each user. To simplify the description, the protocol goes over several iterations, and each iteration includes an initial phase (instead of Phase 1 and Phase 2 in the previous case), a recycling phase where bits that are available as side-information to unintended receivers are sent, and finally, a recursion phase where some linear combinations of previously transmitted signals are fed as new inputs to the same problem. In Case~2, only two feedback realizations could happen captured in Fig.~\ref{Fig:FBCase3}(a) and Fig.~\ref{Fig:FBCase3}(d), and in the recursive step, we send random linear combination of the bits for which no feedback was received. In Case~3, we take advantage of the feedback structure and send individual equations that we know the intended receiver is {\it missing} and rely on the statistics of the channel to make some of these equations available to the other receiver. This way, future iterations will have a shorter combined Phase~1 and Phase~2, which results in higher achievable rates. 

\noindent {\bf Phase~1}: The transmitter creates 
\begin{align}
\frac{m}{1-\delta_{12}}
\end{align}  
linearly independent combinations of the $m$ bits for receiver $1$ and sends them out. When feedback channel realizations $(a)$ and $(c)$ of Fig.~\ref{Fig:FBCase3} occur, which happens with frequency $\left( 1 - \delta \right)$, statistically 
\begin{align}
\label{Eq:Rx1FB}
\underbrace{(1-\delta)}_{\text{realizations a $\&$ c}} \frac{\delta-\delta_{12}}{1-\delta_{12}} m
\end{align} 
combinations are available at ${\sf Rx}_2$ and needed at ${\sf Rx}_1$. {\color{blue} The transmitter creates the same number as given in~\eqref{Eq:Rx1FB} linearly independent combinations of the signals that fell in channel realizations $(a)$ and $(c)$. Denote these new combinations by $v_{1|2}$.  Note that to create these new combinations, the transmitter only needs to know $S_{F2T}[t]$ which is the case in realizations $(a)$ and $(c)$.} Moreover, for $\delta - \delta_{12}$ fraction of the time, feedback realization $(b)$ of Fig.~\ref{Fig:FBCase3} occurs and due to the statistics of the channel, we know 
\begin{align}
\label{Eq:Rx1noFB}
\delta\frac{\delta-\delta_{12}}{1-\delta_{12}} m = \frac{\delta}{1-\delta} \left| v_{1|2} \right|
\end{align} 
combinations are {\it missing} at ${\sf Rx}_1$. Note that a fraction $\left( 1- \delta \right)$ of these combinations is available at ${\sf Rx}_2$. We randomly select a fraction $\delta$ of the combinations that are missing at ${\sf Rx}_1$ when feedback realization $(b)$ of Fig.~\ref{Fig:FBCase3} occurs, and denote them by $v^{\mathrm{noFB}}_{1|2}$. {\color{blue} To Shih-Chun, sorry typo fixed.}

{\color{blue}
\begin{remark}
Here, we would like to point out a subtle but important distinction between combinations in $v_{1|2}$ and in $v^{\mathrm{noFB}}_{1|2}$. In the former, we create random combinations of previously transmitted combinations in Phase~1. Thus, statistically for large $m$, none of these new combinations are known a priori to either of the receivers. In the latter, $v^{\mathrm{noFB}}_{1|2}$, the transmitter selects individual combinations among previously transmitted combinations in Phase~1, and a fraction $\left( 1- \delta \right)$ of these are already known to ${\sf Rx}_2$. We will use the structure of $v^{\mathrm{noFB}}_{1|2}$ to reduce the communication length of the recursive steps as discussed below.
\end{remark}}

\noindent {\bf Phase~2}: Similar to Phase~1 with swapping IDs.

\noindent {\bf Phase~3}: In this phase, the transmitter encodes $v_{1|2}$ and $v_{2|1}$ using erasure codes of rate $(1-\delta)$. Note that $\left| v_{1|2} \right| = \left| v_{2|1} \right|$. The transmitter creates the XOR of the encoded bits for ${\sf Rx}_1$ and ${\sf Rx}_2$ and sends them out. This Phase takes  
\begin{align}
\frac{\left| v_{1|2} \right|}{(1-\delta)} = \frac{(1-\delta_F)(\delta-\delta_{12})}{(1-\delta)(1-\delta_{12})}m \overset{\delta_F = \delta}= \frac{(\delta-\delta_{12})}{(1-\delta_{12})}m.
\end{align} 
time instants. 

\noindent {\bf Recursive step}: The main difference between the achievability strategies of Case~2 and Case~3 lies in the recursive step. In this case, $v^{\mathrm{noFB}}_{1|2}$ and $v^{\mathrm{noFB}}_{2|1}$ unlike Case~2 are not random linear combinations of previously transmitted signals, but rather are the equations that we know the intended receiver is missing. {\color{blue} We note that $|v^{\mathrm{noFB}}_{1|2}| = |v^{\mathrm{noFB}}_{2|1}|$ is given in \eqref{Eq:Rx1noFB}, and due to the specific choice of channel parameters in Case~3, we do not need to recycle bits from realization $(d)$ of Fig.~\ref{Fig:FBCase3}}.  Due to the statistics of the channel, a fraction $(1-\delta)$ of these equations are available to the other receiver. This enables us to reduce the combined length of Phase~1 and Phase~2 in future iterations. More specifically, for the second iteration, instead of having a combined length of
\begin{align}
\label{Eq:LongPhase}
\underbrace{\frac{\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}}}_{\mathrm{Phase~1}} + \underbrace{\frac{\left| v^{\mathrm{noFB}}_{2|1} \right|}{1-\delta_{12}}}_{\mathrm{Phase~2}} = \frac{2\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}},
\end{align}
the transmitter creates
\begin{align}
\label{Eq:ShortenPhase}
\frac{(1+\delta)\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}},
\end{align}
random linear combinations of $v^{\mathrm{noFB}}_{1|2}$ and $v^{\mathrm{noFB}}_{2|1}$ and sends them out {\color{blue} in one ``super-phase'' rather than two separate phases}. Note that receiver ${\sf Rx}_i$ knows a fraction $(1-\delta)$ of $v^{\mathrm{noFB}}_{\bar{i}|i}$ and needs all of $v^{\mathrm{noFB}}_{i|\bar{i}}$, $i=1,2$. Thus, the number of equation provided by (\ref{Eq:ShortenPhase}) enables ${\sf Rx}_i$ to do exactly what could have been accomplished with (\ref{Eq:LongPhase}). {\color{blue} To Shih-Chun: You are right, but this is what the receivers need, we do not claim reception yet. To clarify this, note that without any prior knowledge, each receiver would need
\begin{align}
\frac{\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}},
\end{align}
linearly independent combinations for a total of 
\begin{align}
\frac{2\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}}.
\end{align}
However, $v^{\mathrm{noFB}}_{1|2}$ contains the equations that we know ${\sf Rx}_1$ is missing, and statistically, a fraction $(1-\dl)$ of them are already available at ${\sf Rx}_2$ and a fraction $\dl$ would interfere with ${\sf Rx}_2$. Thus, ${\sf Rx}_2$ only needs a total of 
\begin{align}
\frac{(1+\delta)\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}},
\end{align}
random linear combinations as given in \eqref{Eq:ShortenPhase}}. Following this logic, for the $j^{\mathrm{th}}$ iteration, $j = 2,3,\ldots$, the combined length of Phase~1 and Phase~2 is given by
\begin{align}
\label{Eq:ShortenPhaseIterationj}
\frac{(1+\delta^{j-1})\left| v^{\mathrm{noFB}}_{1|2} \right|}{1-\delta_{12}},
\end{align}
where, with slight abuse of notation, $v^{\mathrm{noFB}}_{1|2}$ is the outcome of iteration $j-1$.


\noindent {\bf Termination}: To simplify the protocol, when the remaining bits in $v^{\mathrm{noFB}}_{1|2}$ and $v^{\mathrm{noFB}}_{2|1}$ is $o\left( m^{1/3} \right)$ we stop the recursion and send the remaining bits using time sharing between the two erasure codes. Note that while we used $o\left( m^{1/3} \right)$ as our termination threshold, any threshold with vanishing (as $m \rightarrow \infty$) impact would work. 

\noindent {\bf Decoding}: Decoding is carried on similar to Case~2. 

\noindent {\bf Achievable rates}: To simplify the calculations, we define
\begin{align}
\eta \overset{\triangle}= \frac{\delta}{(1+\delta)}, 
\end{align}
The total communication time (ignoring $O\left( m^{2/3} \right)$ terms from termination and other approximations discussed in Remark~\ref{remark:Bernstein}) can be then calculated as 
\begin{align}
T & = \underbrace{\frac{2m}{(1-\delta_{12})}}_{\mathrm{ph.~1~}\&\mathrm{~2~of~iteration~1}} + \underbrace{\frac{(\delta-\delta_{12})m}{(1-\delta_{12})}}_{\mathrm{ph.~3~of~iteration~1}} \nonumber \\
& ~+ \underbrace{\frac{(1+\delta)m}{(1-\delta^2)} \frac{\delta(\delta-\delta_{12})}{(1-\delta_{12})}}_{\mathrm{ph.~1~}\&\mathrm{~2~of~iteration~2}} + \underbrace{\frac{(\delta-\delta_{12})m}{(1-\delta_{12})} \frac{\delta(\delta-\delta_{12})}{(1-\delta_{12})}}_{\mathrm{ph.~3~of~iteration~2}} \nonumber \\
& ~+ \underbrace{\frac{(1+\delta^2)m}{(1-\delta^2)} \left(\frac{\delta(\delta-\delta_{12})}{(1-\delta_{12})}\right)^2}_{\mathrm{ph.~1~}\&\mathrm{~2~of~iteration~3}} + \underbrace{\frac{(\delta-\delta_{12})m}{(1-\delta_{12})} \left(\frac{\delta(\delta-\delta_{12})}{(1-\delta_{12})}\right)^2}_{\mathrm{ph.~3~of~iteration~3}} + \ldots \nonumber \\
& \overset{\delta_{12} = \delta^2}= \frac{m}{(1-\delta^2)} \left( 1 + \frac{1}{1-\delta\eta} \right) + \frac{\eta m}{1-\delta \eta} + \frac{\delta^2 \eta m}{(1-\delta^2)} \times \frac{1}{1-\delta^2 \eta} \nonumber \\
& = \frac{m}{1-\delta \eta} \left( \eta + \frac{1}{1-\delta^2} \right) + \frac{m}{1-\delta^2} \left( 1 + \frac{\delta^2 \eta}{1-\delta^2 \eta} \right) \nonumber \\
& = \frac{(1+\delta)m}{1+\delta-\delta^2} \left( \frac{1+\delta-\delta^2}{1-\delta^2} \right) + \frac{m}{1-\delta^2} \left( \frac{(1+\delta)}{1+\delta-\delta^3 \eta} \right) \nonumber \\
& \overset{\eqref{Def:beta-case3}}= \frac{m}{(1-\delta)} + \frac{m}{(1-\delta)\beta} \nonumber \\
& = \frac{(1+\beta)m}{(1-\delta)\beta}.
\end{align}
The achievable rates are then calculated as $R_i = m/T$ which coincide with the expression given in (\ref{Eq:RSUMCase3}). 
\end{comment}

This completes the achievability proof of Case~3 and thus, the proof of Theorem~\ref{THM:Ach_IFB}.

==> Conclusion.tex <==
We studied the throughput region of spatially correlated interference packet networks. We quantified the impact of spatial correlation at the transmitters by deriving an extremal rank-ratio inequality. To achieve the outer-bounds, we developed a new transmission protocol that could have as many as three phases of communication. Our communication protocol takes full advantage of delayed interference structure knowledge and the available spatial correlation side information.  We learned that spatial correlation at the transmitters defines the shape of the throughput region while spatial correlation at the receivers defines the size of this region. 

In this work we assumed that each transmitter starts with a large number of packets to communicate. An interesting direction is to study and to characterize the throughput region for stochastic packet arrival with potential delivery deadlines. % The stability region of the problem can be studied and authors in~\cite{pan2016stability} did so for the results of~\cite{AlirezaInfocom2014}.
